Ground Tests of Einstein's Equivalence Principle: From Lab-based to 10-m Atomic Fountains

To date, no framework combining quantum field theory and general relativity and hence unifying all four fundamental interactions, exists. Violations of the Einstein's equivalence principle (EEP), being the foundation of general relativity, may hold the key to a theory of quantum gravity. The universality of free fall (UFF), which is one of the three pillars of the EEP, has been extensively tested with classical bodies. Quantum tests of the UFF, e.g. by exploiting matter wave interferometry, allow for complementary sets of test masses, orders of magnitude larger test mass coherence lengths and investigation of spin-gravity coupling. We review our recent work towards highly sensitive matter wave tests of the UFF on ground. In this scope, the first quantum test of the UFF utilizing two different chemical elements, Rb-87 and K-39, yielding an E\"otv\"os ratio $\eta_{\,\text{Rb,K}}=(0.3\pm 5.4)\times 10^{-7}$ has been performed. We assess systematic effects currently limiting the measurement at a level of parts in $10^8$ and finally present our strategies to improve the current state-of-the-art with a test comparing the free fall of rubidium and ytterbium in a very long baseline atom interferometry setup. Here, a 10 m baseline combined with a precise control of systematic effects will enable a determination of the E\"otv\"os ratio at a level of parts in $10^{13}$ and beyond, thus reaching and overcoming the performance limit of the best classical tests.

==> input/oldexperiments.tex <==
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
Experiment & A & B  & \EotAB\\
\hline\hline

Palo Alto~\cite{Peters99Nature} & \textsuperscript{133}Cs&SiO$_2$ &$(7.0\pm 7.0)\times 10^{-9}$\\

Paris~\cite{Merlet10Metrologia} & \Rb&SiO$_2$ &$(4.4\pm 6.5)\times 10^{-9}$\\

\hline
M\"unchen~\cite{Fray04PRL} & \Rbb&\Rb &$(1.2\pm 1.7)\times 10^{-7}$\\

Palaiseau~\cite{Bonnin13PRA} & \Rbb&\Rb &$(1.2\pm 3.2)\times 10^{-7}$\\

W\v{u}h\`an~\cite{Zhou15arxiv} & \Rbb&\Rb &$(2.8\pm 3.0)\times 10^{-8}$\\

Firenze~\cite{Tarallo14PRL} & \textsuperscript{87}Sr&\textsuperscript{88}Sr &$(0.2\pm 1.6)\times 10^{-7}$\\

\hline
Hannover~\cite{Schlippert14PRL} & \K&\Rb& $\etav$\\
\hline
\end{tabular}
\end{center}
